Aspire: Practical Batch Queries on Dynamic Encrypted Database with Full Leakage Suppression

Leakage-abuse attacks against encrypted database systems exploit semantic leakage and pose a severe threat to the confidentiality of plaintext data and queries. To address this problem, we propose a zero-leakage encrypted database that rules out leakage-abuse attacks, which fundamentally rely on semantic leakage. We first distinguish between two kinds of zero-leakage security. Ideal zero-leakage forbids the disclosure of any information beyond public parameters, whereas restricted zero-leakage additionally permits the leakage of metadata (such as database size and query timing). We show that restricted zero-leakage is sufficient to thwart leakage-abuse attacks and is achievable in practice. We then formally define adaptive restricted zero-leakage security and present Aspire, an encrypted database that satisfies this notion. Aspire integrates probabilistic batch code and minimal perfect hashing to support efficient batch keyword queries and dynamic updates while revealing only non-semantic metadata. Experimental results demonstrate the practicality and efficiency of Aspire, showing that Aspire can achieve an amortized query latency of less than 1.38 ms (7.53 s for a batch of 5461 keyword queries), with an amortized communication cost of approximately 2.95 KB (16.1 MB in total), on a $2^{22}$ key-value pairs database.

==> Alg_Reconstruct.tex <==
\begin{algorithm}[!t]
    \footnotesize
    \caption{KVPIR.Reconstruct.}
    \label{alg4}
    \SetKwFunction{FMain}{Reconstruct}
    The client and the server run the Reconstruct at a certain predetermined time. The client holds a $MaxCount$, which is initialized as $max(Count)$.
    \SetKwProg{Bn}{procedure}{}{end}
    \Bn{\FMain{}}{
        Client:\\
        \If{$Rcount\%b=0$}{
            $MaxCount=max(Count)$\;
        }
        Downloads the $\widetilde{B}_{Rcount\%b}$ from the server and decrypts it as $DB'$\;
        \For{$(k,i,op)\in S_1[Rcount\%b]$}{
            \eIf{$op$ is ADD}{
                $(v,p)\gets S_2[k]$\;
                Adds $k||v||i$ to $DB'$\;
                $p\gets p-1$\;
                \eIf{$p=0$}{Remove $S_2[k]$\;}{$S_2[k]=(v,p)$\;}
                
            }{
                Deletes the entry starting with $k$ from $DB'$\;
            }
        }
        $S_1[Rcount\%b]\gets \emptyset$\;
        \eIf{$|DB'|\leq MaxCount$}{
            Pads $DB'$ with random value to the size of $MaxCount$\;
        }{  
            Retrieves $|DB'|-MaxCount$ entries from $DB'$ as $DB_{extra}$\;
            \For{$k||v||i\in DB_{extra}$}{
                Adds $(k,i,ADD)$ to $S_1[Rcount\%b]$\;
                \eIf{$S_2[k]\neq \bot$}{
                    $(v,p)\gets S_2[k]$, $S_2[k]=(v,p+1)$\;
                }{
                    $S_2[k]=(v,1)$\;
                }
            }
        }
        Sets $K$ as the keywords in $DB'$, $mph_{Rcount\%b}\gets MPH.Setup(K)$\;
        Rearrange the $DB'$ according to $mph_{Rcount\%b}$\;
        Encrypts $DB'$ as $\widetilde{KV}_{Rcount\%b}$ and uploads it to the server\;
        $Rcount=Rcount+1$\;
        Server:\\
        {\color{blue}
        Runs $\{\widetilde{B}_1,...,\widetilde{B}_{b-1}\}\gets\text{BatchPIR.Setup}(\widetilde{KV}_0,...,\widetilde{KV}_{b-1}\})$\;
        Replaces the reconstructed bucket\;
        $Rcount=Rcount+1$\;
        }
        
    }
    
\end{algorithm}

==> Alg_Reconstruct_server.tex <==
\begin{algorithm}[!t]
    
    \caption{Reconstruct.}
    \label{alg5_server}
    \SetKwFunction{FMain}{Reconstruct}
    {\color{cyan}The server holds a $BSize$ and a $BSize_{old}$, which record the size of the bucket and are initialized as the size of the bucket}\; 
    \SetKwProg{Bn}{procedure}{}{end}
    \Bn{\FMain{}}{
        $\vdots$\\
        Server:\\
        {\color{cyan}
        \If{$Rcount\%b=0$}{
            $BSize_{old}\gets BSize$\;
            $BSize\gets |\widetilde{KV}'_{Rcount\%b}|$\;
            \If{$BSize>BSize_{old}$}{
                \Comment{The size of the database grows}\;
                Pads the $\widetilde{KV}_i$ to the size of $BSize$ for all $i\in \{1,...,b\}$\;
            }
        }
        \If{$BSize<BSize_{old}$}
        {
            \Comment{The database shrinks}\;
            Pads the $\widetilde{KV}'_{Rcount\%b}$ to the size of $BSize_{old}$\;
        }
        $\widetilde{KV}_{Rcount\%b}\gets \widetilde{KV}'_{Rcount\%b}$\;
        \If{$Rcount\%b=b-1$ and $BSize<BSize_{old}$}{
            Remove the paddings in $\widetilde{KV}_{i}$ for all $i \in \{0,...,b\}$\;
        }
        $Rcount=Rcount+1$\;
        }
    }
    
\end{algorithm}

==> Alg_Update.tex <==
\begin{algorithm}[!t]
    \footnotesize
    \caption{KVPIR.Update.}
    \label{alg3}
    \SetKwFunction{FMain}{Update}
    The client holds a $S_1=\{s_0,...,s_{b-1}\}$, where $s_i$ is initialized as empty, a $S_2$, which stores the updated key-value pairs and is initialized as empty, a $Count=\{c_0,...,c_{b-1}\}$, which records the real size of each bucket. The server and the client both hold a $Rcount$, which records the reconstruction times and is initialized as 0\;
    \SetKwProg{Bn}{procedure}{}{end}
    \Bn{\FMain{$k,v,op$}}{
        Client:\\
        Computes $Pos={pos_1,...,pos_p}$, where $pos_i$ is $hash_i(k)$\;\Comment{$hash_i$ is the $i$th hash function in PBC}\;
        \eIf {$op$ is ADD}{
            $S_2[k]=(v,p)$\; \Comment{The $p$ represents there $p$ buckets to reconstruct before deleting this entry from $S_2$}\;
            \For{$i \in [p]$}{
                Adds $(k,i,ADD)$ to $S_1[pos_i]$, if $(k,i,DEL)\in S_1[pos_i]$, delete $(k,i,DEL)$ from $S_1[pos_i]$\;
                $c_i\gets c_i+1$\;
            }
        }{
            \For{$i \in [p]$}{
                Adds $(k,i,DEL)$ to $S_1[pos_i]$, if $(k,i,ADD)\in S_1[pos_i]$, delete $(k,i,ADD)$ from $S_1[pos_i]$\;
                $c_i\gets c_i-1$\;
            }
        }
    }
    
\end{algorithm}
